Automated Side Channel Analysis of Media Software with Manifold Learning

The prosperous development of cloud computing and machine learning as a service has led to the widespread use of media software to process confidential media data. This paper explores an adversary's ability to launch side channel analyses (SCA) against media software to reconstruct confidential media inputs. Recent advances in representation learning and perceptual learning inspired us to consider the reconstruction of media inputs from side channel traces as a cross-modality manifold learning task that can be addressed in a unified manner with an autoencoder framework trained to learn the mapping between media inputs and side channel observations. We further enhance the autoencoder with attention to localize the program points that make the primary contribution to SCA, thus automatically pinpointing information-leakage points in media software. We also propose a novel and highly effective defensive technique called perception blinding that can perturb media inputs with perception masks and mitigate manifold learning-based SCA. Our evaluation exploits three popular media software to reconstruct inputs in image, audio, and text formats. We analyze three common side channels - cache bank, cache line, and page tables - and userspace-only cache set accesses logged by standard Prime+Probe. Our framework successfully reconstructs high-quality confidential inputs from the assessed media software and automatically pinpoint their vulnerable program points, many of which are unknown to the public. We further show that perception blinding can mitigate manifold learning-based SCA with negligible extra cost.

==> alluppermath-notations.tex <==
%{math-notations}

% natural numbers
\newcommand{\NATURALS}{{\rm Nat}}

% functions names inside of math environment
\newcommand{\fun}[1]{\hbox{\it #1\/}}

% brackets that surround syntax (as in denotational semantics)
\newcommand{\synbracket}[1]{[\![{#1}]\!]}

% logic
\newcommand{\IFF}{\Leftrightarrow}
\newcommand{\DEF}{\stackrel{{\rm def}}{=}}
\newcommand{\DEFEQUIV}{\stackrel{{\rm def}}{\equiv}}
\newcommand{\DEFIFF}{\stackrel{{\rm def}}{\IFF}}

% lambda calculus
\newcommand{\LAMBDA}[1]{\lambda{#1}\:.\:}
\newcommand{\FREEVARS}[1]{{\it FV\/}\synbracket{#1}}	% free variables
\newcommand{\FREEIDS}[1]{{\it FreeIds\/}(#1)}	% free identifiers
\newcommand{\SYNTAXWITHFOR}[3]{[#2/#3]#1}	% subst #2 for #3 in #1
\newcommand{\WITHFOR}[3]{#1[#2/#3]}		% subst #2 for #3 in #1
\newcommand{\BETAREDUCESTO}{\stackrel{\beta}{\Rightarrow}}
\newcommand{\ETAREDUCESTO}{\stackrel{\eta}{\Rightarrow}}
\newcommand{\DELTAREDUCESTO}{\stackrel{\delta}{\Rightarrow}}
\newcommand{\BETAEQUALS}{\stackrel{\beta}{=}}
\newcommand{\ETAREQUALS}{\stackrel{\eta}{=}}
\newcommand{\DELTAEQUALS}{\stackrel{\delta}{=}}

% higher order lambda calculus
\newcommand{\POLY}[1]{\Lambda{#1}\:.\:}
\newcommand{\ALLTYPE}[1]{\forall{#1}\:.\:}
\newcommand{\EXISTSTYPE}[1]{\exists{#1}\:.\:}
\newcommand{\DEPFUNTYPE}[1]{\Pi{#1}\:.\:}
\newcommand{\DEPSUMTYPE}[1]{\Sigma{#1}\:.\:}

% recursion theory
\newcommand{\ZEROORMORE}[1]{{#1}^{\rm *}}
\newcommand{\ONEORMORE}[1]{{#1}^{+}}

% category theory
\newcommand{\DOM}[1]{{\it Domain\/}(#1)}
\newcommand{\POWERSET}[1]{{\it PowerSet\/}(#1)}

% topology
\newcommand{\CLOSURE}[1]{\overline{#1}}
\newcommand{\LUB}{{\rm lub}}			% least upper bound

% set theory
\def\elem{\hbox{\raise.13ex\hbox{$\scriptstyle\in$}}}
\newcommand{\GRAPH}{{\it graph}}

% relations
\newcommand{\RELATIONTYPE}[1]{2^{(#1)}}


==> calculation.tex <==
% $Id: calculation.tex 2 2008-12-23 22:46:05Z gary.leavens $
%
% Calculational proofs, a la Dijkstra, Gries, Back and von Wright, etc.
% See: David Gries, "Teaching Calculation and Discrimination:
%      A More Effective Curriculum", CACM 34(3):44-55, Mar. 1991.
% and
%      Ralph-Johan Back and Joakim von Wright,
%      "Refinement Calculus: A Systematic Introduction",
%      Springer-Verlag, 1998.
%
% AUTHOR: Gary T. Leavens

% EXAMPLES
%
% A simple example of the use of these macros is as follows.
%
% \begin{calculation}
% \FORMULA{\vec{RD}}
% \EQREASON{definition of $\vec{RD}$}
% \FORMULA{(RD_1, \ldots, RD_j, \ldots, RD_{12})}
% \REASON{\sqsubseteq}{$F_j$ is monotonic}
% \FORMULA{(RD_1, \ldots, F_j(\vec{RD}), \ldots, RD_{12})}
% \EQREASON{definition of $\vec{RD'}$}
% \LASTFORMULA{\vec{RD'}}
% \end{calculation}
%
% The following is a slightly more advanced example.
%
% \begin{calculation}
% \FORMULA{F(\vec{RD'}) \sqsubseteq \FOCUS{F^n(\vec{\emptyset})}}
% \EQREASON{assumption $F^n(\vec{\emptyset}) = F^{n+1}(\vec{\emptyset})$}
% \FORMULA{F(\vec{RD'}) \sqsubseteq \FOCUS{F^{n+1}(\vec{\emptyset})}}
% \EQREASON{definition of iteration of a function}
% \FORMULA{F(\vec{RD'}) \sqsubseteq F(F^n(\vec{\emptyset}))}
% \REASON{\impliedby}{monotonicity of $F$}
% \FORMULA{\vec{RD'} \sqsubseteq F^n(\vec{\emptyset})}
% \REASON{\impliedby}{transitivity}
% \FORMULA{\vec{RD'} \sqsubseteq F(\vec{RD})
%         \wedge F(\vec{RD}) \sqsubseteq F^n(\vec{\emptyset})}
% \EQREASON{assumption $F(\vec{RD}) \sqsubseteq F^n(\vec{\emptyset})$}
% \FORMULA{\vec{RD'} \sqsubseteq F(\vec{RD})}
% \REASON{\impliedby}{Lemma~7}
% \QEDFORMULA{\vec{RD} \sqsubseteq F(\vec{RD})}
% \end{calculation}
%
% An much more sophisticated example, with subdeductions a la Back and
% von Wright is the following.
%
% \begin{calculation}
% \FORMULA{\alpha(\{tr: (z, \ell') \mid tr \in \gamma(RD_k)\}) }
% \EQREASON{definition of $\alpha$}
% \FORMULA{\{(x, SRD(tr')(x))
%              \mid x \in \textrm{dom}(tr')
%                   \wedge tr' \in \{tr: (z, \ell') \mid tr \in \gamma(RD_k)\} \} }
% \EQREASON{set theory
%          ($tr'$ ranges over $tr: (z, \ell')$ for $tr \in \gamma(RD_k)$)}
% \FORMULA{\{(x, SRD(tr: (z, \ell'))(x))
%              \mid x \in \textrm{dom}(tr: (z, \ell')),
%                    \FOCUS{tr \in \gamma(RD_k)} \} }
% \EQREASON{definition of $\gamma$}
% \FORMULA{\{(x, SRD(tr: (z, \ell'))(x))
%              \mid x \in \textrm{dom}(tr: (z, \ell')),
%                (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}}
% \EQREASON{set theory}
% \FORMULA{
%     \begin{array}{rl}
%         \{(x, SRD(tr: (z, \ell'))(x)) &
%              \mid x \neq z, x \in \textrm{dom}(tr: (z, \ell')), \\
%              & ~ (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \} \\
%         \cup \:
%         \{(x, SRD(tr: (z, \ell'))(x)) &
%              \mid x = z, x \in \textrm{dom}(tr: (z, \ell')), \\
%              & ~ (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}
%     \end{array}
%         }
% \EQREASON{focusing on the second set}
% \SUBDEDUCTION{
%      \begin{array}{rl}
%         \{(x, SRD(tr: (z, \ell'))(x)) &
%              \mid x = z, x \in \textrm{dom}(tr: (z, \ell')), \\
%              & ~ (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}
%      \end{array}
%        }
%   \EQREASON{set theory}
%   \FORMULA{\{(z, \FOCUS{SRD(tr: (z, \ell'))(z)}) 
%              \mid z \in \textrm{dom}(tr: (z, \ell')),
%                (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \} }
%   \EQREASON{definition of $SRD$}
%   \FORMULA{\{(z, \ell') 
%              \mid \FOCUS{z \in \textrm{dom}(tr: (z, \ell'))},
%                (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k)
%              \} }
%   \EQREASON{definition of $\textrm{dom}$}
%   \FORMULA{\{(z, \ell') 
%              \mid (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \} }
%   \EQREASON{definition of $\gamma$}
%   \FORMULA{\{(z, \ell') \mid tr \in \gamma(RD_k) \} }
%   \EQREASON{$tr$ can be constructed by writing the pairs of
%              $\gamma(RD_k)$ in some order}
%   \FORMULA{\{(z, \ell') \} }
% \CONCLUDE{
%    \begin{array}{l}
%     \begin{array}{rl}
%         \{(x, SRD(tr: (z, \ell'))(x)) &
%              \mid x \neq z, x \in \textrm{dom}(tr: (z, \ell')), \\
%              & ~ (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}
%     \end{array} \\
%     \cup \: \{(z, \ell')\}
%    \end{array}
%     }
% \EQREASON{focusing on the first set}
% \SUBDEDUCTION{
%     \begin{array}{rl}
%         \{(x, SRD(tr: (z, \ell'))(x)) &
%              \mid x \neq z, x \in \textrm{dom}(tr: (z, \ell')), \\
%              & ~ (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}
%      \end{array}
%        }
%   \EQREASON{definition of $SRD$}
%   \FORMULA{\{(x, SRD(tr)(x))
%              \mid x \neq z, x \in \textrm{dom}(tr), 
%               (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}}
%   \EQREASON{set theory and the range of $SRD$}
%   \FORMULA{\begin{array}{l}
%              \{(x, SRD(tr)(x))
%                       \mid x \in \textrm{dom}(tr), 
%               (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \} \\
%            \setminus \: \{(z, \ell) \mid \ell \in \Lab\}
%            \end{array}
%           }
%   \EQREASON{Lemma \ref{lemma:simplifyToRD}}
%   \FORMULA{RD_k \setminus \{(z, \ell) \mid \ell \in \Lab\}}
% \LASTCONCLUDE{(RD_k \setminus \{(z, \ell) \mid \ell \in \Lab\})
%            \cup \{(z, \ell')\}}
% \end{calculation}


%%%%%%% The macros themselves follow %%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% You may want to define the following with \renewcommand...

% Brackets around normal and fixed width reasons
\newcommand{\LEFTREASONBRACKET}{\langle}
\newcommand{\RIGHTREASONBRACKET}{\rangle}
% Brackets for long reasons
\newcommand{\LONGLEFTREASONBRACKET}{\left\LEFTREASONBRACKET}
\newcommand{\LONGRIGHTREASONBRACKET}{\right\RIGHTREASONBRACKET}
% width of long and fixed width reasons
\newcommand{\LONGREASONWIDTH}{5.4in}
\newcommand{\FIXEDWIDTHREASONWIDTH}{\LONGREASONWIDTH}
% The phrase that starts each reason
\newcommand{\BYPHRASE}{by~}
% Provability symbol
\newcommand{\PROVABILITYSYMBOL}{\vdash}
% Has type symbol
\newcommand{\CALCULATIONHASTYPE}{:}
% Subdeduction symbols a la Back and von Wright
\newcommand{\SUBDEDUCTIONMARKER}{\bullet}
\newcommand{\CONCLUDEMARKER}{\cdot}

% The macros below assume that you have defined \QED,
% e.g., as \newcommand{\QED}{q.e.d.}


%%% The rest shouldn't usually need to be redefined

% The main environment
\newenvironment{calculation}{
\samepage
\begin{tabbing}
n \= n \= n \= n \= mm \= n \= mm \= n \= mm \= n \= mm \= n \= mm \= \kill
}{
\end{tabbing}
}

% Use for the last formula (to avoid extra vertical space)
\newcommand{\LASTFORMULA}[1]{\> \ensuremath{#1}}
% Use for the last formula in a proof that concluses the proof
\newcommand{\QEDATEND}{~~\QED}
\newcommand{\QEDFORMULA}[1]{\LASTFORMULA{#1\QEDATEND}}

% All other formulas in a calculation
\newcommand{\FORMULA}[1]{\LASTFORMULA{#1} \\}

% Generic reason, with connective and the justification
\newcommand{\REASON}[2]{%
    \ensuremath{#1}\> \>
       \mbox{\ensuremath{\LEFTREASONBRACKET}{\BYPHRASE}#2\ensuremath{\RIGHTREASONBRACKET}} \\}

% Reasons with longer justifications, with the right bracket at the end
\newcommand{\FIXEDWIDTHREASON}[2]{%
     \ensuremath{#1}\> \>
       \ensuremath{\LEFTREASONBRACKET}{\BYPHRASE}%
       \parbox[t]{\FIXEDWIDTHREASONWIDTH}{#2\ensuremath{\RIGHTREASONBRACKET}}
       \\
     }

% Reasons with longer justifications, with big brackets around the reason
\newcommand{\LONGREASON}[2]{%
    \ensuremath{#1}\> \>
      \ensuremath{\LONGLEFTREASONBRACKET
                  \parbox[c]{\LONGREASONWIDTH}{{\BYPHRASE}#2}
                  \LONGRIGHTREASONBRACKET
                 }
      \\
    }

% Specialization of reasons to equality
\newcommand{\EQREASON}[1]{\REASON{=}{#1}}
\newcommand{\EQLONGREASON}[1]{\LONGREASON{=}{#1}}
\newcommand{\EQFIXEDWIDTHREASON}[1]{\FIXEDWIDTHREASON{=}{#1}}

% Use \FOCUS{E} to say that subformula E will be changed in the following step
\newcommand{\FOCUS}[1]{\mbox{``}#1\mbox{''}}


%% The following are for Back and von Wright style calculations.
%% First time users may want to ignore these.

% Use for assumptions in a type-deduction style proof
\newcommand{\GIVEN}[1]{\FORMULA{#1}}
% Use \PROVETHAT to start the body of a type-deduction style proof.
\newcommand{\PROOFLINE}[2]{\ensuremath{#1} \> \ensuremath{#2} \\}
\newcommand{\PROVETHAT}[1]{\PROOFLINE{\PROVABILITYSYMBOL}{#1}}
%% Subdeductions
% Use to start a subdeduction
\newcommand{\SUBDEDUCTION}[1]{\+\+\kill\PROOFLINE{\SUBDEDUCTIONMARKER}{#1}}
% Use to separate one subdeduction from another
\newcommand{\ANDALSO}{\-\-\kill}
% Use to start the next subdeduction after \ANDALSO
\newcommand{\NEXTDEDUCTION}[1]{\PROOFLINE{\SUBDEDUCTIONMARKER}{#1}}
% Use to conclude a subdeduction 
\newcommand{\CONCLUDE}[1]{\-\-\kill\PROOFLINE{\CONCLUDEMARKER}{#1}}
% Use when the last formula is also a conclusion
\newcommand{\LASTCONCLUDE}[1]{\-\-\kill\ensuremath{\CONCLUDEMARKER} \> \ensuremath{#1}}
% Use in a type-deduction proof instead of \REASON, to give the rule name
\newcommand{\TYPINGRULE}[1]{\ensuremath{\CALCULATIONHASTYPE} \> ~~~ #1 \\}

% end of calculation.tex


==> denotational-semantics.tex <==
% requires math-notations

% Typography as in Schmidt's book: Denotational Semantics.
% Many of the following defs must be used in a math environment; all can be.

% natural numbers: \NATURALS
\renewcommand{\NATURALS}{{\it Nat}}
\newcommand{\ZERO}{{\it zero}}
\newcommand{\ONE}{{\it one}}
\newcommand{\TWO}{{\it two}}
\newcommand{\THREE}{{\it three}}
\newcommand{\FOUR}{{\it four}}
\newcommand{\PLUS}{{\it plus}}
\newcommand{\MINUS}{{\it minus}}
\newcommand{\TIMES}{{\it times}}
\newcommand{\EQUALNATURALS}{{\it equals}}

% integers: \INTEGER
\newcommand{\INTEGER}{{\it Int}}
\newcommand{\ADDR}{{\it Addr}}

% Booleans: \BOOLEAN
\newcommand{\BOOLEAN}{{\it Boolean}}
\newcommand{\TRUE}{{\it true}}
\newcommand{\FALSE}{{\it false}}
\newcommand{\NOT}{{\it not}}
\newcommand{\OR}{{\it or}}
\newcommand{\AND}{{\it and}}
\newcommand{\IFEXP}[3]{#1 \rightarrow #2 [\!] #3 }
\newcommand{\IFHEAD}[1]{#1 \rightarrow}
\newcommand{\IFELSE}{[\!]~}

% truth values
\newcommand{\TR}{{\it Tr}}
\newcommand{\TT}{{\it tt}}
\newcommand{\FF}{{\it ff}}

% Strings: \STRING
\newcommand{\STRING}{{\it String}}
\newcommand{\EMPTYSTRING}{{\it empty}}
\newcommand{\ERRORSTRING}{{\it error}}
\newcommand{\CONCATSTRINGS}{{\it concat}}
\newcommand{\LENGTHOFSTRING}{{\it length}}
\newcommand{\SUBSTRING}{{\it substr}}		% 3 arguments

% other primitive domains
\newcommand{\UNIT}{{\it Unit}}
\newcommand{\ERROR}{{\it Error}}

% other standard semantics domain names
\newcommand{\ANSWERS}{{\it Answer}}
\newcommand{\CMDCONT}{{\it Cmdcont}}
\newcommand{\DENOTABLE}{\mbox{\it Denotable-value}}
\newcommand{\ENVIRONMENT}{{\it Environment}}
\newcommand{\EXPRESSIBLE}{\mbox{\it Expressible-value}}
\newcommand{\EXPCONT}{{\it Expcont}}
\newcommand{\LOCATION}{{\it Location}}
\newcommand{\PROCEDURE}{{\it Procedure}}
\newcommand{\REFERENCE}{{\it Reference}}
\newcommand{\RESULT}{{\it Result}}
\newcommand{\STORE}{{\it Store}}
\newcommand{\STORABLE}{\mbox{\it Storable-value}}
\newcommand{\UNBOUND}{{\it Unbound}}
\newcommand{\VALUE}{{\it Value}}

% disjoint union: $A + B$
\newcommand{\INJECTION}[1]{{\rm in}\!{#1}}
\newcommand{\ISTEST}[1]{{\rm is}\!{#1}}
\newcommand{\CASEHEAD}[1]{\mbox{{\bf cases} ${#1}$ {\bf of} }}
\newcommand{\CASE}[2]{{#1} \:\rightarrow\: {#2}}
\newcommand{\CASESEP}{[\!]}
\newcommand{\CASEELSE}{\mbox{{\bf else} }}
\newcommand{\CASEEND}{{\bf end}}

% product space: $A \times B$
\newcommand{\PAIR}[2]{({#1},{#2})}
\newcommand{\FST}{{\it fst}}
\newcommand{\SND}{{\it snd}}
\newcommand{\ATINDEX}[2]{#1 \downarrow #2}
% Note $\ZEROORMORE{A} = Unit + A + (A \times A) + (A \times A \times A) + ...$
% Lists are $Unit + A + (A \times A) + (A \times (A \times A)) + ...$

% list space: $\LIST{A}$
\newcommand{\LIST}[1]{{\it List}(#1)}
\newcommand{\LNIL}{{\it nil}}
\newcommand{\LCONS}{{\it cons}}
\newcommand{\LHEAD}{{\it hd}}
\newcommand{\LTAIL}{{\it tl}}
\newcommand{\LNULL}{{\it null}}

% function space: $A \rightarrow B$
\newcommand{\UPDATEFUN}[3]{[{#1} \mapsto {#2}]{#3}}

% finite functions
\newcommand{\FINITEARROW}{\stackrel{{\rm fin}}{\rightarrow}}

% lifted domain: $\LIFT{A}$
\newcommand{\LIFT}[1]{{#1}_{\bot}}
\newcommand{\STRICTLAMBDA}[1]{\underline{\lambda}{#1}\:.\:}
\newcommand{\LETHEAD}[2]{\mbox{{\bf let} }{#1} = {#2}\mbox{ {\bf in} }}
\newcommand{\MAP}[2]{\mbox{{\bf map} }{#1} => {#2\{#1\}}}

% fixpoints
\newcommand{\FIX}{{\it fix}}

% common valuation functions
\newcommand{\MEANING}[2]{{\cal #1}\synbracket{#2}}
\newcommand{\DENEXPRESSION}[1]{\MEANING{E}{#1}}
\newcommand{\DENCOMMAND}[1]{\MEANING{C}{#1}}
\newcommand{\DENLITERAL}[1]{\MEANING{L}{#1}}
\newcommand{\DENPROGRAM}[1]{\MEANING{P}{#1}}

% an environment for typesetting
\newenvironment{DENOTATIONAL}{%
\samepage
\begin{tabbing}
mmm \= mmm \= mmm \= mmm \= mmm \= mmm \= mmm \= mmm \= \kill
}{
\end{tabbing}
}


==> framework.tex <==
\section{Model Architecture}
\label{sec:framework}
We now report the architecture and parameters of our framework. The
$Enc_{trace}$ of VAE-LP module is reported in \T~\ref{tab:vae-trace}.
$Enc_{image}$ and $Dec_{image}$ are reported in \T~\ref{tab:vae-image}. The
generator $G$ and discriminator $D$ of our GAN module are listed in
\T~\ref{tab:gan-G} and \T~\ref{tab:gan-D}, respectively.

\begin{table*}[!htp]
	\centering
	\small
	\caption{The image encoder $Enc_{image}$ and image decoder
    $Dec_{image}$ architectures.}
	\label{tab:vae-image}
	\begin{tabular}{|c|c|c||c|c|c|}
		\hline
		\multicolumn{3}{|c||}{Image Encoder} & \multicolumn{3}{c|}{Image Decoder}\\ \hline
		Layer & Act. & Output shape & Layer & Act. & Output shape\\ \hline
		Input & - & $3 \times 128 \times 128$ & Input & - & $128 \times 1 \times 1$  \\ 
		Conv $4 \times 4_{/2,1}$ & LReLU(0.2) & $128 \times 64 \times 64$ & Deconv $4 \times 4_{/1,0}$ & BN + ReLU & $128 \times 4 \times 4$\\ 
		ResBlock~\cite{he2016deep} & - & $128 \times 64 \times 64$  & ResBlock & - & $128 \times 4 \times 4$\\
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $128 \times 32 \times 32$ & Deconv $4 \times 4_{/2,1}$ & BN + ReLU & $128 \times 8 \times 8$\\
		ResBlock & - & $128 \times 32 \times 32$ & ResBlock & - & $128 \times 8 \times 8$\\
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $128 \times 16 \times 16$ & Deconv $4 \times 4_{/2,1}$ & BN + ReLU & $128 \times 16 \times 16$\\
		ResBlock & - & $128 \times 16 \times 16$ & ResBlock & - & $128 \times 16 \times 16$\\
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $128 \times 8 \times 8$ & Deconv $4 \times 4_{/2,1}$ & BN + ReLU & $128 \times 32 \times 32$\\
		ResBlock & - & $128 \times 8 \times 8$ & ResBlock & - & $128 \times 32 \times 32$\\ 
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $128 \times 4 \times 4$ & Deconv $4 \times 4_{/2,1}$ & BN + ReLU & $128 \times 64 \times 64$\\
		ResBlock & - & $128 \times 4 \times 4$ & ResBlock & - & $128 \times 64 \times 64$\\
		Conv $4 \times 4_{/1,0}$ & LReLU(0.2) & $128 \times 1 \times 1$ & Deconv $4 \times 4_{/2,1}$ & Tanh & $3 \times 128 \times 128$\\
		Output & - & $128$ & Output & - & $3 \times 128 \times 128$\\
		\hline
	\end{tabular}
\end{table*}

\begin{table*}[!htp]
	\centering
	\small
	\caption{The trace encoder $Enc_{trace}$ architecture.}
	\label{tab:vae-trace}
	\begin{tabular}{|c|c|c|}
		\hline
		\multicolumn{3}{|c|}{Trace Encoder} \\ \hline
		Layer & Act. & Output shape \\ \hline
		Input & - & $3 \times 512 \times 512$  \\ 
		Normalize & - & $3 \times 512 \times 512$ \\ 
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $64 \times 256 \times 256$ \\
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $64 \times 128 \times 128$ \\
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $64 \times 64 \times 64$ \\
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $128 \times 32 \times 32$ \\
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $256 \times 16 \times 16$ \\
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $512 \times 8 \times 8$ \\
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $512 \times 4 \times 4$ \\
		Conv $4 \times 4_{/1,0}$ & BN + Tanh & $128 \times 1 \times 1$ \\
		Output & - & $128$ \\
		\hline
	\end{tabular}
\end{table*}

\begin{table*}[!htp]
	\centering
	\small
	\caption{The generator $G$ architecture.}
	\label{tab:gan-G}
	\begin{tabular}{|c|c|c||c|c|c|}
		\hline
		\multicolumn{3}{|c||}{Encoder} & \multicolumn{3}{c|}{Decoder}\\ \hline
		Layer & Act. & Output shape & Layer & Act. & Output shape\\ \hline
		Input & - & $3 \times 128 \times 128$ & Input & - & $1024 \times 1 \times 1$  \\ 
		Conv $4 \times 4_{/2,1}$ & - & $128 \times 64 \times 64$ & Deconv $4 \times 4_{/2,1}$ & BN + ReLU & $1024 \times 2 \times 2$\\ 
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $256 \times 32 \times 32$ & Deconv $4 \times 4_{/2,1}$ & BN + ReLU & $1024 \times 4 \times 4$\\
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $512 \times 16 \times 16$ & Deconv $4 \times 4_{/2,1}$ & BN + ReLU & $1024 \times 8 \times 8$\\
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $1024 \times 8 \times 8$ & Deconv $4 \times 4_{/2,1}$ & BN + ReLU & $512 \times 16 \times 16$\\
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $1024 \times 4 \times 4$ & Deconv $4 \times 4_{/2,1}$ & BN + ReLU & $256 \times 32 \times 32$\\
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $1024 \times 2 \times 2$ & Deconv $4 \times 4_{/2,1}$ & BN + ReLU & $128 \times 64 \times 64$\\
		Conv $4 \times 4_{/2,1}$ & LReLU(0.2) & $1024 \times 1 \times 1$ & Deconv $4 \times 4_{/2,1}$ & Tanh & $3 \times 128 \times 128$\\
		Output & - & $1024 \times 1 \times 1$ & Output & - & $3 \times 128 \times 128$\\
		\hline
	\end{tabular}
\end{table*}

\begin{table*}[!htp]
	\centering
	\small
	\caption{The discriminator $D$ architecture.}
	\label{tab:gan-D}
	\begin{tabular}{|c|c|c|}
		\hline
		\multicolumn{3}{|c|}{Discriminator} \\ \hline
		Layer & Act. & Output shape \\ \hline
		Input & - & $3 \times 128 \times 128$  \\ 
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $128 \times 64 \times 64$ \\
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $256 \times 32 \times 32$ \\
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $512 \times 16 \times 16$ \\
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $1024 \times 8 \times 8$ \\
		Conv $4 \times 4_{/2,1}$ & BN + LReLU(0.2) & $1024 \times 4 \times 4$ \\
		Conv $4 \times 4_{/1,0}$ & Sigmoid & $1 \times 1 \times 1$ \\
		Output & - & $1$ \\
		\hline
	\end{tabular}
\end{table*}


==> grammar.tex <==
%{grammar}, needs {obey}

%\newcommand{\heading}[1]{\vspace{3ex}{\noindent#1}\vspace{1.5ex}}
\newcommand{\goesto}{\mbox{$::=$}}
\newcommand{\arbno}[1]{#1\hbox{\rm*}}
\newcommand{\nonterm}[1]{\mbox{$\langle$#1$\rangle$}}

\newenvironment{grammar}{
  \def\:{\goesto{}}
  \def\|{$\vert$}
  \tt \myobeycr%
  \begin{tabbing}%
  \qquad \= $\vert$ \= \qquad \= \kill%
}%
{\unskip\end{tabbing}}

\newenvironment{grammar*}{
  \def\:{\goesto{}}
  \def\|{$\vert$}
  \tt%
  \begin{tabbing}%
  \qquad \= $\vert$ \= \qquad \= \kill%
}%
{\unskip\end{tabbing}}

\newenvironment{roman-grammar}{
  \def\:{\goesto{}}
  \def\|{$\vert$}
  \myobeycr%
  \begin{tabbing}%
  \qquad \= $\vert$ \= \qquad \= \hspace*{5cm} \= \qquad \= \kill%
}%
{\unskip\end{tabbing}}

\newenvironment{roman-grammar*}{
  \def\:{\goesto{}}
  \def\|{$\vert$}
  \begin{tabbing}%
  \qquad \= $\vert$ \= \qquad \= \hspace*{5cm} \= \qquad \= \kill%
}%
{\unskip\end{tabbing}}

\newenvironment{mathGrammar}{
  \def\:{\goesto{}}
  \def\|{\hbox{$\vert$}}
   \begin{displaymath}%
     \tt \obeyspaces%
}%
{\unskip\end{displaymath}}

% Commented grammars

% length before comments start on right
\newlength{\BEFOREGRAMCOMMENTLEN}
\setlength{\BEFOREGRAMCOMMENTLEN}{7cm}

% style of text inside quotations
\newcommand{\GRAMCOMMENTSTYLE}[1]{\texttt{#1}}

\newenvironment{commented-grammar}{%
\begin{grammar}%
\qquad \= $\vert$ \= \qquad \hspace*{\BEFOREGRAMCOMMENTLEN} \= \kill%
}{%
\end{grammar}%
}

\newcommand{\gramcomment}[1]{\textrm{``\GRAMCOMMENTSTYLE{#1}''}}


==> implementation.tex <==
\section{Implementation}
\label{sec:implementation}

% In addition to the standard inputs of table data supported by the popular
% \vfl\ frameworks~\cite{vfl}, we also spend extra engineering efforts to
% implement a convolutional neural network (CNN) layer, and therefore, the
% \vfl\ framework can take images as the inputs. This way, we are able to
% comprehensively study the potential attack vectors of \vfl\ models with respect
% to conventional table data and high-dimensional inputs.
\subsection{Model Architecture}

One encoder for cacheline, pagetable and cachebank. Three decoders for image data,
audio data and text data correspondingly.

\subsection{Datasets}

Image data: 1) CelebA, 2) ChestX-ray8 (chest X-ray images of eight common thoracic diseases).

Audio data: 1) SC09 (human sound clips of saying number from 0 to 9, with identity
of the speakers annotated.), 2) sub-URMP, which contains audio clip of instrument
and is widely used for cross modal generation (since reconstructing human sounds in
the wild is very chanllenging, it's better to try simple dataset. We can state that
``features'' of the audio is reconstructed.).

Text data: 1) COCO Caption (we can state that information is very ``dense'' in this
dataset, since the sentences are densely composed of named entities, verbs and relatives),
2) Enron Email Dataset (the text lib is word-level, so passwords can NOT be processed by
the lib.).

==> motivation.tex <==
\section{Adversarial Dominating Inputs in VFL}
\label{sec:adi}

This section formulates adversarial dominating inputs (ADIs) in the context of
VFL. To this end, we first define the threat model as follows.

\smallskip
\noindent \textbf{Threat Model.}~It is consistently assumed by the vertical
federated-learning scenarios that clients are \textit{honest but curious}. For
instance, in a two-party case (see \F~\ref{fig:background}), those two parties
are non-colluding and one is compromised by an adversary. We assume that the
adversary can learn data only from the client that it corrupted; however, not
data from the host will be disclosed to the adversary on the client.

From a holistic perspective, adversarial dominating inputs denote a set of
inputs that once being fed and processed by one client, will dominate the
prediction and make other clients' contribution negligible. Rigorously, we
specify \adi\ as follows. 


==> notes-for-recording.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      NOTE: This is just an outline         %
%      with some random thoughts             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Related Work}
\label{sec:related}

~\cite{bengio2013representation} Various AEs.
%
As soon as there is a notion of ``representation'', one can think of a manifold by considering the
variations in input space which are captured by or reflected (by corresponding changes) in the 
learned representation.
%
To first approximation, some directions are well preserved (the tangent directions of the manifold),
while others are not (directions orthogonal to the manifolds). With this perspective, the primary 
unsupervised learning task is then seen as modeling the structure of the data-supporting manifold.
%
The associated representation being learned can be associated with an intrinsic coordinate system on the
embedded manifold.
%

~\cite{li2017unsupervised} Extracting behavior information from speech.
%
Manifold in the couples therapy domain.
%
In this behavioral manifold we expect similar behaviors to appear closer together than they do in the
original signal space.

~\cite{holden2015learning} Projecting invalid or corrupt motion onto the manifold for removing error.
Projection and inverse projection can be used to fix corrupted motion data.
%
\textbf{Filling in Missing Data.}

~\cite{Fu_2015_CVPR} The rich intrinsic structure, i.e. semantic manifold, of the semantic
categories in the embedding space.
%
No manually defined ontology is required and the space is learned using a vast unannotated
data.

~\cite{radford2015unsupervised} To understand the landscape of the latent space. Walking
in this latent space results in semantic changes to the image (such as objects being added
and removed.).

~\cite{zhu2016generative} It is easy to “fall off” the manifold of natural images while
editing. Conventional methods, low-level principles. NN, capture higher-level
information about natural images. Stays on, or close to, the natural image manifold.
%
Generative models of local image statistics have long been used as a prior for image
restoration problems such as image denoising and deblurring.
%
Approximates the image manifold by learning a model using GAN from a large-scale image collection.
%
The Euclidean distance in the latent space often corresponds to a perceptually meaningful visual
similarity.

~\cite{shen2020interpreting} Latent space is the semantic space. For face images, varibales
in latent space control face attributes.

Geometric understanding of deep learning.

Manifold assumption: \textit{natural high dimensional data concentrates close
to a non-linear low-dimensional manifold.} Suppose all $C \time W \times H$ images are
photos of faces, and randomly choosing values from $[0, 255]$ for pixels will not
get such images, so we hope we could find a subset of all possible choices. Manifold
hypothesis states that this subset lives in an ambient space of lower dimension $N$, 
where $N$ is much smaller than the origianl dimension, i.e., $255^{C \times W \times H}$.

How the method can be interpreted?
Cross modal generation? 
Or transfering from ``side channel'' domain data to image /audio/text domain data?
In other words, we can treat the side channel trace as an another representation of the original data?

A data-driven unified framework for detecting SCA-vulnerable codes of \ms by first
learning a reconstruction mapping between the data ``observed'' in side channel domain and data
from origianl domain. When training this mapping, a low-dimensional joint manifold of the data 
in both domains is implicitly learned, capturing a highly expressive representation
that is robust to noise and other input perturbations~\cite{zhu2018image}.
 

An important thing to discuss is the difference between how lib and NN treate media data. Libs treate meida data
as matrix of float points, but NN treat meida data as lots of ``content''.

Autoencoder (AE) on manifold learning. Encoder learns the map from high-dimensional
data to low-dimensional manifold. Decoder is inverse to encoder.

Comparison with genSCA. Generative model is a special case of AE.

\section{Proposed Method}
\label{sec:method}

\subsection{Attack}

perceptual learning archetype

between domain projection

We take a step back -- from a generative model to a simple autoencoder, which
is composed of a trace encoder and data type based decoders, namely, image decoder,
audio decoder and text decoder in our setting.

Pointwise loss complemented with a discriminator in GANs. We also give a definition of
``privacy'' as follows. For face images, the ``privacy'' is the identity of the person,
and for audio clips of human sound, ``privacy'' includes the content of the auido clip
and the indentity of the speaker. However, the ``privacy'' is not ``intendedly touched'' in the training
process, so we add privacy-based constraints, e.g. when training the audio decoder,
discriminator also works as a classifier for speakers' indentities to force the reconstructed
audios contain the identities of the speakers.

Text decoder is slightly different with image/audio decoder. Instead of directly generating
a sentence from the \fixme{embedded} vector of side channel trace, a sentence is generated word by word,
more specificly, each word is generated based on the side channel trace with the aid of
the previous word. The text decoder captures the dependency between words.

\subsection{Detecting}

We reuse the trace encoder proposed in genSCA, but add attention module in the encoder.
1) fast convergency, 2) localize the vulnerable code blocks

\subsection{Defence}

From one of the following aspects: 1) the inherent error of NN, or 2) \textit{decoder} is
a piecewise linear approximation of the map from low-dimensional manifold to high-dimensional data.




==> obey.tex <==
%{obey}

% \myobeycr is same as \obeycr, but doesn't do a \@gobblecr.
{\catcode`\^^M=13 \gdef\myobeycr{\catcode`\^^M=13 \def^^M{\\}}%
\gdef\restorecr{\catcode`\^^M=5 }}

% \obeytabs
{\catcode`\^^I=13 \gdef\obeytabs{\catcode`\^^I=13 \def^^I{\hbox{\hskip 4em}}}}

% \obeyspaces
{\obeyspaces\gdef {\hbox{\hskip0.5em}}}

% environment for displayed text, indented, obeys cr, tab, spaces
\newenvironment{obeyDisplay}{%
\samepage%
\begin{list}{}{}\item\obeyspaces\obeytabs\obeycr}{%
\end{list}}


==> summary.tex <==
\section{Summary of Changes}

The reviewers wanted to see the following changes addressed in the resubmission:

\begin{enumerate}
\item Improve description of the threat model and potential attack scenarios.

\item Evaluate on more and different systems (different CPUs) also with
  additional noise to demonstrate noise resilience and also noise introduced by
  mitigations/real workload.

\item From the open-source implementation[0], it seems like PIN is directly used
  instead of a real-world attack. But what happens if we remove data points from
  the traces instead of writing them to "0"? Not sure how/if the noise was added
  on the input? Noise should be: leave cache hits out false cache hits (might
  occur with low probability) wrong order of the cache hits. While this could be
  covered by the evaluated Gaussian noise, the paper lacks to describe this
  first step (data collection) and argumentation about real-world noise.

\item Provide a showcase of the attack traces with a real cache attack in a
  userspace-only scenario, i.e., collect cache traces via (Flush+Reload,
  Prime+Probe, etc.) and evaluate that data.

\item Provide the representation of cache-side channel traces and how they are
  fed into the encoding step (for instance,
  <_Z14pipe_interfacePP8HunspelliP8_IO_FILEPc>:": 564, -> is used as input for
  the network). While it is possible to guess it is transformed into a matrix,
  but there is no description about that.

\item An evaluation of the end-to-end demonstration.

\end{enumerate}

%\vspace*{-20pt}
%
\smallskip
\noindent \textbf{Summary Response:}~We thank the reviewers for the constructive
comments and meta-reviews. During revisions, we have addressed each of these
required changes. We have performed many more experiments, and have incorporated
the results of these new experiments in our discussions. We believe that the
revised paper addresses the gaps identified in the original version, and thus
provides more comprehensive insights on how our attack can be launched in an
``end-to-end'' userspace-only scenario, and its promising resilience toward
various noisy scenarios. In the following section we supply a point-by-point
response to the list of comments in the Major Revision decision, and summarize
other changes we have made to the manuscript.
\\\\
\noindent \textit{1. Required changes in meta-review: Improve description of the
  threat model and potential attack scenarios.}

\noindent \textbf{Response:}~Thank you for the advice.
In \textbf{Threat Model and Attack Scenarios} on Page 2, we have revised our
threat model, research assumption, and how side channels are acquired by
attackers.
\\\\
\noindent \textit{2a. Required changes in meta-review: Evaluate on more and
  different systems (different CPUs).}

\noindent \textbf{Response:}~We launch \pp\ attack on both Intel Xeon CPU and
AMD Ryzen CPU. Our evaluation is presented in \S~\ref{subsec:real-world}.
\\\\
\noindent \textit{2b. evaluate with additional noise to demonstrate noise
  resilience and also noise introduced by mitigations/real workload.}

\noindent \textbf{Response:}~We benchmarked in total \textbf{nine} different
noise insertion schemes. This includes three schemes to perturb side channel
traces logged by Pin, and three schemes to perturb cache side channels logged by
\pp\ (as suggested in the meta-review \textit{3a}). We launch \pp\ attack by
pinning the victim process (e.g., \libjpeg) and the \spy\ process on the same
CPU core. Therefore, we benchmark three real workloads by launching 1) a
\texttt{bzip2} software on the same core, 2) another victim process processing a
different input on the same core, and 3) another victim process processing the
same input on the same core. Note that since we have three \ms, the
aforementioned nine noise insertion schemes actually lead to \textbf{27}
settings. Our attack manifests reasonably high accuracy across nearly all
settings. See our evaluation in \S~\ref{subsec:noise} and \appx~\ref{sec:noise}.

As for \textit{noise introduced by mitigations}, we use Oblivious RAM
(PathOHeap) to mitigate our attack. PathOHeap can effectively mitigate our
attack, although its incurred extra cost is very high; please refer to
\S~\ref{subsec:oram}. \\\\
\noindent \textit{3a. what happens if we remove data points from the traces
  instead of writing them to "0"? Not sure how/if the noise was added on the
  input? Noise should be: leave cache hits out false cache hits (might occur
  with low probability) wrong order of the cache hits}

Thank you for the suggestion. Yes, we have benchmarked these different noise
insertion schemes and give discussions accordingly. Please see our response to
\textit{2b}.
\\\\
\noindent \textit{3b. While this could be covered by the evaluated Gaussian
  noise, the paper lacks to describe this first step (data collection) and
  argumentation about real-world noise}

Thank you for the comment. We clarified how side channel traces are collected
using either Pin or launching \pp\ attack in \S~\ref{subsec:real-world} and
\appx~\ref{subsec:real-attack-details}. As aforementioned, we benchmarked three
noise introduced by real-world workloads in \S~\ref{subsec:noise}.
\\\\
\noindent \textit{4. Provide a showcase of the attack traces with a real cache
  attack in a userspace-only scenario, i.e., collect cache traces via
  (Flush+Reload, Prime+Probe, etc.) and evaluate that data}

We benchmark userspace-only scenarios where attackers can launch
\pp\ attack~\cite{Tromer10} to log cache activities when \ms\ is processing a
secret input. We use Mastik~\cite{yarom2016mastik}, a micro-architectural
side-channel toolkit, to launch ``out-of-the-box'' \pp\ and log victim's L1I and
L1D cache activities. We pin victim process and \spy\ process on the same CPU
core; see attack details in \S~\ref{subsec:real-world} and
\appx~\ref{subsec:real-attack-details}.
\\\\
\noindent \textit{5. Provide the representation of cache-side channel traces and
  how they are fed into the encoding step.}

Thank you for pointing this out. We use \appx~\ref{sec:input} to clarify this
point. Particularly, \F~\ref{fig:input} gives a holistic view on how side
channel traces, collected from either Pin or \pp\ attack, are transformed into a
matrix and then fed into our encoder. We also give analysis on the noise
resilience due to our trace representation and encoder design in
\appx~\ref{sec:input}. \\\\
\noindent \textit{6. An evaluation of the end-to-end demonstration.}

As aforementioned, we launch an end-to-end attack to benchmark userspace-only
scenarios where attackers can launch \pp\ attack~\cite{Tromer10} to log cache
activities when \ms\ is processing a secret input. We use
Mastik~\cite{yarom2016mastik}, a micro-architectural side-channel toolkit, to
launch ``out-of-the-box'' \pp\ and log victim's L1I and L1D cache activities. We
pin victim process and \spy\ process on the same CPU core; see attack details in
\S~\ref{subsec:real-world} and \appx~\ref{subsec:real-attack-details}.
\\\\
\noindent \textit{``[...] If the trace data collected from an actual side-channel
  attack is too noisy to reproduce the original media.''}

We report promising quantitative results (attack \libjpeg) in
\S~\ref{subsec:real-world}. We further present quantitative and qualitative
results in \appx~\ref{subsec:real-attack-details}. We note that attack results
are generally promising; the recovered media data still manifest encouraging
visual similarity compared with the reference inputs. Please see
\S~\ref{subsec:real-world} and \appx~\ref{subsec:real-attack-details} for our
results and discussions.
\\\\
\noindent \textit{``[...] or if the time to collect all the needed trace data using
  only side-channel attacks is too long''}

\smallskip
\noindent \textbf{Trace Collection and Training Cost.}~For the newly-added
\pp\ attack evaluation, to collect traces for training, we spend 54 hours for
\libjpeg, 36 hours for \ffmpeg, and 100 hours for \hunspell. Note that if we
exclude the time used for processing data and saving the data into the accepted
format of Pytorch (i.e., Tensor), the remaining time cost is 9 hours, 12 hours,
27 hours for \libjpeg, \ffmpeg\ and \hunspell, respectively. This remaining time
cost primarily includes multiple rounds of \pp\ and model training duration.
Overall, the ``training phases'' using cache side channels collected by \pp\ can
likely take \textit{several hours to a few days}~\cite{Zhang12}. That is, we
interpret that our approach spends reasonable amount of training effort. Please
refer to paragraph \textbf{Running Time} in
\appx~\ref{subsec:real-attack-details} for discussions.

\smallskip
\noindent \textbf{Unknown Input Generation Cost.}~It takes less than 10 seconds
to reconstruct 2,000 media inputs (40 batches), using our well-trained
autoencoder. Therefore, for a well-trained autoencoder, the ``generation phase''
is usually not a concern.

\smallskip
\noindent \textbf{Victim Software Slowdown Caused by \pp.}~We report slowdown
when launching \pp\ attack in \T~\ref{tab:pp} and present corresponding
discussions in paragraph \textbf{Workload} in
\appx~\ref{subsec:real-attack-details} and in \S~\ref{subsec:real-world}.
%
We note that launching \pp\ attack over \ms, though slows down its execution, is
still reasonable (within 500ms). In all, three \ms\ attacked in this research is
much complex than crypto algorithms like AES. Their frequent memory accesses can
lead to many cache miss during \pp. Nevertheless, two \ms\ take on average less
than 100ms to process a confidential input (under \pp), whereas the most complex
\ms, \ffmpeg, takes less than 500ms to process a voice recording under \pp. We
interpret the results as reasonable and comparable to previous \pp\ attacks
launched toward crypto libraries~\cite{Tromer10}.

\section{Formatting \& Writing \& Code Release}


\noindent \textit{Paper title.}

\noindent \textbf{Response.}~We slightly tweak our paper title from \textit{Side
  Channel Analysis of Media Software with Manifold Learning} into
\textit{Automated Side Channel Analysis of Media Software with Manifold
  Learning}. We wish to highlight that our attack, fault localization, and
mitigation, are automated.
\\\\
\noindent \textit{Formatting and paper length.}

\noindent \textbf{Response.}~We clarify that during the Revise phase we have
performed many new experiments and added many new results and corresponding
discussion. This has added quite a number of extra pages to the manuscript.
According to USENIX Security '22 call for paper, ``\textit{all paper
  submissions, including Major Revisions, should be at most 13 typeset pages,
  excluding bibliography and well-marked appendices.}'' We tried our very best
to polish the paper and formatting, move contents to Appendices without
primarily undermining the readability of the first 13 pages. If accepted, we
commit to provide an extended version to move all Appendices to the main content
to further ease the reading.
\\\\
\noindent \textit{Major improvement on writing.}

\noindent \textbf{Response.}~We also did an extensive improvement on the
writing, including the grammar, phrasing, and punctuation. In addition, 
edits were made to further improve the flow and readability of the paper. We
reconstructed some sentences to address over complex structures, and also
removed some redundant, repetitive or unnecessary phrases.
\\\\
\noindent \textit{Code and dataset release.}

\noindent \textbf{Response.}~Instead of using the Github anonymous service which
was not stable, we release our artifact at
\url{https://github.com/research-artifact/manifold-sca}. Our results can be
reproduced from the released codebase automatically. Looking ahead, we will
clean the codebase and provide more documents. We commit to maintain our
codebase for results verification and benefit follow up research in this field.

\section{Other Review Comments}

\noindent \textit{Review~\#404A: The authors should clarify whether this (bug
  localization) is performed manually or using an automated approach.}

\noindent \textbf{Response.}~Thank you very much for your interest in this
research and all the kind words. We have clarified that we automatically
localize buggy assembly instructions and then manually map assembly code into
source code in the third paragraph of \S~\ref{subsec:design-attention}.
\\\\
\noindent \textit{Review~\#404A: To make the results reproducible the authors
  should additionally mention learning rate, batch size, convergence criteria,
  early stopping, dropout etc.}

\noindent \textbf{Response.}~We have added those information in
\S~\ref{subsec:implementation}. As we explained in
\S~\ref{subsec:implementation}, the training ends after 100 epochs. We did not
use early stopping because it may end the training at undesired local optimum.
We also did not use dropout because the logged side channel trace is very
sparse. \\\\
\noindent \textit{Review~\#404A: Furthermore, it seems that cache banks in this
  form are not used in the L1 anymore, which I think should be mentioned.} 

\noindent \textbf{Response.}~In \S~\ref{sec:attack}, we have clarified that we
use Intel Pin to log memory access traces and then convert them into
corresponding side channel traces, including cache bank traces. 
\\\\
\noindent \textit{Review~\#404A: I would also suggest adding a sentence each
  that the resolution when performing attacks on those components is 4B,64B, and
  4096B.}

\noindent \textbf{Response.}~Thank you for the suggestion. We have added that in
\S~\ref{sec:attack}.
\\\\
\noindent \textit{Review~\#404A: The paper misses an explanation of how the
  traces were taken and on which system. This would be helpful to reproduce the
  results. Please provide more details about how this was performed.}

\noindent \textbf{Response.}~We have clarified this point in \textbf{Threat
  Model and Attack Scenarios} on Page 2 of the paper. We also elaborate on
attack setup in \appx~\ref{sec:attack-appendix} and
\appx~\ref{subsec:real-attack-details}.
\\\\
\noindent \textit{Review~\#404A: I would suggest adding some short summary about
  the framework design before starting directly with 4.1. Same for 6.1 Side
  Channel Attack, 6.3.1.}

\noindent \textbf{Response.}~Thank you for the suggestion. We have added a short
paragraph at each place in the paper.
\\\\
\noindent \textit{Review~\#404A: For Figure 4 I would suggest not using coloring
  to illustrate the green cross, since readers might only print it in
  black/white. Instead, another symbol might be used to highlight the
  corresponding data point.}

\noindent \textbf{Response.}~Thank you for the suggestion. We are using
different symbols in that figure to enhance the readability.
%\noindent \textit{Review~\#404A: In Figure 5, I would suggest also highlighting
%  the terms for the sake of completeness.}
%
%\noindent \textbf{Response.}~Thank you for the suggestion. \fixme{XXX}
%\\\\
%\noindent \textit{Review~\#404A: For the tables 11,14 I would also add a column
%  with the row names.}
%
%\noindent \textbf{Response.}~Thank you for the suggestion. \fixme{XXX}
\\\\
\noindent \textit{Review~\#404A: The community benefits from open-sourcing
  frameworks and results.}

\noindent \textbf{Response.}~Thank you for all the kind words. We fully agree
with you. As mentioned above, we will clean our codebase, add more documents,
and maintain this tool for results verification and benefit follow-up research
in the community.
\\\\
\noindent \textit{Review~\#404A: Nitpicks \& Stylistic}

\noindent \textbf{Response.}~Thank you for all the suggestions. We have fixed
those typos in the paper. We also thank you for the comment on ``stylistic''. We
fully agree that it will save some time to read the paper. In revision we tried
this scheme to mention the first author et. al.; however, it seems not
formatting-friendly as we are tight with 13 pages. If accepted (and therefore we
have 18 pages in total), we promise to use this scheme to ease the reading. 
\\\\
\noindent \textit{Review~\#404A: The authors should clarify whether the code
  localization is performed manually or using an automated approach. If it is an
  automated approach, it should be discussed in more details.}

\noindent \textbf{Response.}~We have clarified that we automatically localize
buggy assembly instructions and then manually map assembly code into source code
in the third paragraph of \S~\ref{subsec:design-attention}.
\\\\
\noindent \textit{Review~\#404A: Section 5 (Attack Setup) should be explained in
  more details and the above mentioned points about cache banks should be
  clarified.}

\noindent \textbf{Response.}~We have clarified this point in \textbf{Threat
  Model and Attack Scenarios} on Page 2 of the paper. We also elaborate on
attack setup in \appx~\ref{sec:attack-appendix} and
\appx~\ref{subsec:real-attack-details}.
\\\\
\noindent \textit{Review~\#404A: Add the numbers and explanations which are
  asked for in the questions.}

\noindent \textbf{Response.}~The above questions have been fixed. 
\\\\
\noindent \textit{Review~\#404A: I would love to see more and different systems
  being evaluated. Furthermore, it would be interesting how the performance is
  on a system with real-world noise in the cloud to additionally verify the
  noise resilience.}

\noindent \textbf{Response.}~As answered to ``meta-review'' comments, we have
evaluated cache side channels logged by \pp\ attack on Intel and AMD CPUs. We
have also benchmarked in total nine noise insertion schemes over all three \ms,
including three real-world workloads launched during \pp\ attack. We present
results in \S~\ref{subsec:real-world} and \S~\ref{subsec:noise}.
\\\\
\noindent \textit{Review~\#404A: Please provide more details about how the
  traces were taken and on which system.}

\noindent \textbf{Response.}~We have clarified this in \S~\ref{sec:attack}.
\\\\
\noindent \textit{Review~\#404A: How is mode collapse considered/prevented in
  the architecture?}

\noindent \textbf{Response.}~We clarified that in paragraph \textbf{Ablation
  Evaluations} in \appx~\ref{sec:case}.
\\\\
\noindent \textit{Review~\#404A: How large is the coefficient beta required to
  be?}

\noindent \textbf{Response.}~We require that $\beta \gg \alpha$ and $\alpha +
\beta = 1$. We have clarified this point in \S~\ref{subsec:design-defense}.
\\\\
\noindent \textit{Review~\#404A: Is it possible to determine the exact size
  required to be able to successfully perform blinding?}

\noindent \textbf{Response.}~Users only need to use one perception blinding. We
have clarified this in the second paragraph of \S~\ref{subsec:design-defense}.
\\\\
\noindent \textit{Review~\#404A: Why is the accuracy increase overall between
  cache bank and cache line only a few percent?}

\noindent \textbf{Response.}~Higher-resolution side channels enable
reconstruction of more vivid images, this does not necessarily promote privacy
stealing. We have clarified this point in \S~\ref{subsubsec:eval-quantitative}.
\\\\
\noindent \textit{Review~\#404A: Please provide more details about the
  side-channel traces. I would also like to see the runtime numbers (n,stddev)
  for the SCAs.} 

\noindent \textbf{Response.}~We have clarified that side channel traces are
logged using Intel Pin in \S~\ref{sec:attack} and the \textbf{Threat Model and
  Attack Scenarios} paragraph on Page 2. For those traces logged using Pin, we
report the runtime numbers in \T~\ref{tab:data-statistics}. When performing new
experiments using \pp, we evaluated both Intel Xeon CPU and AMD Ryzen CPU. For
those traces logged by \pp, we have reported the runtime numbers in
\T~\ref{tab:pp-trace-statistics}.
\\\\
\noindent \textit{Review~\#404A: Please also provide numbers about the runtime
  of the training phase and the runtime of the tests.}

\noindent \textbf{Response.}~We have reported this information in
  \T~\ref{tab:data-statistics} (for experiments based on Pin-logged traces) and
  \T~\ref{tab:pp-trace-statistics} (for experiments based on \pp-logged
  traces).
\\\\
\noindent \textit{Review~\#404A: In the quantitative evaluation, what were the
  number of samples and runs to achieve the 99.9\% confidence score?}

\noindent \textbf{Response.}~Training details of those Face++ APIs are not
disclosed. We elaborate on evaluation setups and leveraged tools,
including Face++, in paragraph \textbf{Tools Used in Evaluations} in
\appx~\ref{sec:attack-appendix}.
\\\\
\noindent \textit{Review~\#404A: How is the autoencoder enhanced to flag the
  side channel logs?}

\noindent \textbf{Response.}~We use the standard attention mechanism. We have
extended \S~\ref{subsec:design-attention}, particularly, the third paragraph, to
clarify the usage of attention and how buggy code is localized.
\\\\
\noindent \textit{Review~\#404A: Were the results responsibly disclosed to the
  affected software developers?}

\noindent \textbf{Response.}~Yes. We give discussions in the last paragraph
\textbf{Confirmation with the Developers} of \S~\ref{subsec:eval-localization}.
\\\\
\noindent \textit{Review~\#404A: How could the side channel be mitigated?}

\noindent \textbf{Response.}~In addition to the perception blinding proposed in
this work, we also benchmark using Oblivious RAM to mitigate our attack in
\S~\ref{subsec:oram}.
%\\\\
%\noindent \textit{Review~\#404B: Regarding the listed six weaknesses.}
%
%\noindent \textbf{Response.}~We thank Review~\#404B for these comments and
%pointing out the weakenesses. To clarify the potential confusion: while we don't
%give a point-to-point response to the ``weaknesses'', we give responses in
%answering your comments below which should cover the ``weaknesses''.
\\\\
\noindent \textit{Review~\#404B: I would recommend introducing clearly in the
  Introduction what is meant by media software.}

\noindent \textbf{Response.}~Thank you for the suggestion. We have extended
\S~\ref{sec:introduciton} with this information.
\\\\
\noindent \textit{Review~\#404B: Hence, this is the first comprehensive study of
  media software to assess how their inputs, which represent private user data,
  could be leaked via SCA. -> Maybe be more precise, comprehensive is difficult
  to quantify}

\noindent \textbf{Response.}~Thank you for the suggestion. We have revised this
sentence as ``This is the first study toward \ms\ of various input formats to
assess how their inputs, which represent private user data, can be leaked via
SCA in a fully automatic way.''
\\\\
\noindent \textit{Review~\#404B: Please provide more clear threat model. If the
  attacker has access to the victim's hardware, I would assume there are simpler
  attacks to do? Why consider accessed cache line, cache bank, or page table
  entries and not some other side-channels?}

\noindent \textbf{Response.}~We have extended the last paragraph of
\textbf{Threat Model and Attack Scenarios} on Page 2 to clarify this point. We
clarify that we aim to demonstrate the effectiveness of our manifold
learning-based attack over commonly used side channels. This way, the attack is
shown as practically approachable, indicating its high impact and threats in
real-world scenarios. \\\\
\noindent \textit{Review~\#404B: we provide a throughout study...-> thorough
  study?}

\noindent \textbf{Response.}~Thank you. We have changed it.
\\\\
\noindent \textit{Review~\#404B: It is also shown that data of same class (e.g.,
  face photos) generally lies in the same manifold, whereas data of different
  classes (face vs. vehicle photos) concentrate on separate manifolds in the
  low-dimensional space [94]. -> Did the authors manage to observe this? (that
  data of the same class)}

\noindent \textbf{Response.}~Yes. We have added a new figure to illustrate this
phenomenon. Please refer to a new Appendix section, \appx~\ref{sec:misc}, on
our empirical exploration of manifold hypothesis.
\\\\
\noindent \textit{Review~\#404B: We first construct a joint, perception-level
  connection...-> Please provide more details as it is not clear what is the
  perception-level connection}

\noindent \textbf{Response.}~We have revised that statement with a new footnote.
\\\\
\noindent \textit{Review~\#404B: We also assume that the entire joint dataset
  formed by the ith media input and the corresponding ith observation lies in a
  joint manifold -> shouldn't this be a part of the threat model? What would
  happen if the assumption is violated? How likely is that the assumption can be
  violated?}

\noindent \textbf{Response.}~We have revised that statement and accordingly
clarified in our ``threat model'' paragraph: we assume that side channel
observations must depend on the inputs of \ms. \\\\
\noindent \textit{Review~\#404B: Please provide details about the architecture
  in the paper (Conv2D blocks). I am curious if the authors explored various
  architectures?}

\noindent \textbf{Response.}~We have elaborated on the model architectures in
\appx~\ref{sec:input}. We give discussion on autoencoder's decent noise
resilience, and analyzed relatively low noise resilience of other neural
architectures in the last paragraph of \appx~\ref{sec:input}.
\\\\
\noindent \textit{Review~\#404B: OK, but wouldn't this depend on the input data
  dimensionality? If the data starts as low-dimensional, 32 dimensions can be a
  lot.}

\noindent \textbf{Response.}~Thank you for pointing this out. We have clarified
that this configuration is decided according to the input data dimensionality in
the \textbf{Encoder $\phi_{\theta}$} paragraph of \S~\ref{subsec:design-attack}.
\\\\
\noindent \textit{Review~\#404B: Our preliminary study (see Fig. 16 in Appendix)
  shows that such explicit metrics suffer from “over-smoothing,” a well-known
  problem that leads to quality degradation of the reconstructed data. -> Maybe
  provide a reference?}

\noindent \textbf{Response.}~Thank you for the suggestion. We have
  provided references for that point.
\\\\
\noindent \textit{Review~\#404B: Another popular approach is to assess the
  “semantics similarity” of reconstructed i0 and reference input i. -> Please
  provide some reference}

\noindent \textbf{Response.}~Thank you for the suggestion. We have revised that
statement and provided references accordingly.
\\\\
\noindent \textit{Review~\#404B: Inspired by advances in program neural
  smoothing [89,90] and SCA based on generative models [51, 81, 108, 111], -> I
  did a brief check and it does not seem all these works use generative models
  (some use discriminative only)}

\noindent \textbf{Response.}~We apologize for this mistake. We have changed the
statement as ``[...] and SCA based on neural networks''.
\\\\
\noindent \textit{Review~\#404B: ``Which logged side channel records contribute
  most to the reconstruction of media data?'' -> OK, so the question is on the
  level of records (i.e., side-channel traces) and not features in those
  traces?}

\noindent \textbf{Response.}~This question is a bit unclear to us. Each trace
contains multiple records. We pinpoint some records on the trace that primarily
contribute to input reconstruction. At that particular statement, we added a
pointer to \appx~\ref{sec:input} to clarify the trace representation with
discussions and figures.
\\\\
\noindent \textit{Review~\#404B: An attention module (we follow the design in
  [105]) is inserted within every two stacked CNN layers. -> Please provide some
  details about the attention module. Also, did the authors try different
  setups?}

\noindent \textbf{Response.}~We follow the design in~\cite{woo2018cbam}, because
it is simple and effective. We have clarified this in \S~\ref{subsec:design-attention}.
% \\\\
% \noindent \textit{Review~\#404B: As a recommendation, it seems to me that
%   section 4.3 would fit better if put closer to the experiments on
%   countermeasures. Now, the reader needs to remember details from quite some
%   pages ago.}
% 
% \noindent \textbf{Response.}~\fixme{TODO: done}
\\\\
\noindent \textit{Review~\#404B: OK, does this mean that this countermeasure is
  not useful for standard side-channel attacks? How difficult would it be to
  combine with some other countermeasures? What happens if the attacker trains
  with the dataset that includes logs with countermeasure?}

\noindent \textbf{Response.}~Thank you for these questions. We have added two 
paragraphs, \textbf{Application Scope} and \textbf{``White-box'' Attackers}, in
\appx~\ref{sec:blind-appx} to discuss this point. We have also evaluated
another popular countermeasure, ORAM, in \S~\ref{subsec:oram}. ORAM can mitigate
our attack, but it incurs high cost and is thus impractical.
\\\\
\noindent \textit{Review~\#404B: Figure 7 would require a bit more discussion as
  it is not trivial to understand what is happening there. Also, the values on
  axes are not readable without a serious zoom}

\noindent \textbf{Response.}~Thank you for these questions. We have moved this
figure to Appendix (\F~\ref{fig:audio}). We put it cross two columns to enhance
the readability. We also give more discussions for this figure.
\\\\
\noindent \textit{Review~\#404B: In general, the authors provide quite a lot of
  tables/figures presenting the results. Unfortunately, I did not notice a lot
  of deeper discussion about the results for many of those.}

\noindent \textbf{Response.}~Thank you for pointing this out. Given that we
evaluated three \ms\ and in total six datasets, we have to present a
considerable number of figures/tables to illustrate the quantitative and
qualitative results. On the other hand, these evaluations and our efforts
provide encouraging results that the proposed attack is, as expected,
\textit{agnostic} to particular \ms\ implementation and media data format, and
can be launched fully automatically toward real-world software. In general,
promising results are \textit{consistently} observed for all settings. We view
this as an advantage of our approach.

In revision, we have added and extended several Appendix sections to discuss
evaluation setup (\appx~\ref{sec:attack-appendix} and
\appx~\ref{subsec:real-attack-details}), results analysis (\appx~\ref{sec:case}
and \appx~\ref{subsec:real-attack-details}), and discussion on noise resilience
(\appx~\ref{sec:input}). 
\\\\
\noindent \textit{Review~\#404B: Given the reconstructed voice commands (number
  0–9), we train two classifiers for speaker identity and command 0–9
  classification [86]. -> There are no details about those two classifiers in
  the paper.}

\noindent \textbf{Response.}~Thank you for pointing this out. We have added
clarifications in the \textbf{Quantitative Evaluation} paragraph of
\appx~\ref{sec:attack-appendix}. We added a footnote at that particular statement
to point to \appx~\ref{sec:attack-appendix}.
\\\\
\noindent \textit{Review~\#404B: In addition, we also identified functions in
  other image transformation routines (e.g., MCU, unsampling) and output dumping
  routines to leak confidential inputs. We manually inspected the corresponding
  implementation of libjpeg and confirmed our findings. -> It would be nice to
  see some more details, at least in the appendix. What exactly is done, how are
  the findings confirmed?}

\noindent \textbf{Response.}~In \appx~\ref{sec:case}, the \textbf{Vulnerable
  Code} paragraph, we present vulnerable code fragments of \libjpeg\ and
\hunspell\ and give discussions. Overall, we manually analyzed how inputs are
propagated into certain program variables, and how those program variables are
used to access memory (and further lead to side channels).
\\\\
\noindent \textit{Review~\#404B: For the mitigation strategy, qualitative
  evaluation says $alpha$ makes a difference, while quantitative says
  $alpha$ makes no notable influence. Could the authors discuss these
  perspectives and provide some recommendations? I do not see details about the
  values for $beta$?}

\noindent \textbf{Response.}~We clarify that $\alpha$ makes no major influence
in masking images, but it makes notable influence in masking text. We clarify
the reasons in detail in the first two paragraphs of
\S~\ref{subsubsec:mitigation-qualitative}. Also, in revision, we have clarified
that we require $\beta \gg \alpha$ and $\alpha + \beta = 1$ in
\S~\ref{subsec:design-defense}.
%\fixme{TODO: for continuous data, alpha makes
%\fixme{no notable} difference, this is because the privacy (e.g., 
%ID for a face photo) is contributed by all perception contents and mitigation
%is performed on the level of perception contents. The privacy is \fixme{not}
%simply a sum of all perception contents (i.e., they are \textit{not} linearly
%correlated). But for discrete data (i.e., text), the privacy is the
%word-dependency and we directly mitigate the word-dependency, and as a result,
%the privacy leakage has \textit{notable} change when $\alpha$ increases.}
\\\\
\noindent \textit{Review~\#404B: I am a bit lost about the point of Section 7.
  It feels like missing some introduction. }

\noindent \textbf{Response.}~We have re-organized the structure and put that
``Section 7'' as a subsection of our evaluation. It evaluates noise resilience of our attack.
\\\\
\noindent \textit{Review~\#404B: The overall matching rates are high, which
  largely outperforming the baseline — random guess. -> outperform the baseline
  (or high, largely outperforming the baseline)}

\noindent \textbf{Response.}~Thank you; we have fixed it.
\\\\
\noindent \textit{Review~\#404B: I find Table 14 to be a bit too vague to
  provide a proper indication of the generalization ability. Could we see
  results for other types of input?}

\noindent \textbf{Response.}~In revision, we provide qualitative results in
\F~\ref{fig:cifar100} in \appx~\ref{sec:case}. Overall, ``generalization'' is a
limitation of our manifold learning-based approach due to the manifold learning
hypothesis. We also discussed potential enhancement on generalization in the
\textbf{Generalization} paragraphs of \appx~\ref{sec:case}.
\\\\
\noindent \textit{Review~\#404B: Interesting division of countermeasures into SW
  and HW based. What happens when we have the same countermeasure realized in SW
  and HW (which can often happen, depending on target)? }

\noindent \textbf{Response.}~We agree that should effectively mitigate our
attack. Indeed, only using ORAM (SW-based mitigation) can provably mitigate
quite a number of side channels, including our attack (as shown in
\S~\ref{subsec:oram}). We would like to assess various well-known HW/SW
mitigations in front of our automated attack (in a cross-architecture setting)
as full exploration for future work of this paper. We also compared HW- and
SW-based approaches in the revised related work section.
%\\\\
%\noindent \textit{Review~\#404B: Why is ORAM example important to be singled
%  out?}
%
%\noindent \textbf{Response.}~ORAM denotes an effective 
\\\\
\noindent \textit{Review~\#404B: Any indications for future work or limitations
  of this work?}

\noindent \textbf{Response.}~We have mentioned that ``generalization'' is a
primary limitation of this work. Inspired by recent works~\cite{Weber2021},
leveraging our framework to launch automated assessment of microarchitectural
differences that potentially generate (and amplify) side channels would be
interesting. We mentioned this in \S~\ref{subsec:real-world}. As aforementioned,
we have already released our codebase and all data
at~\url{https://github.com/research-artifact/manifold-sca} for results
verification and also benefit follow-up research from the community.
\\\\
\noindent \textit{Review~\#404B: how does the manifold learning-based attack
  work if there are some other countermeasures (i.e., more common ones)
  implemented?}

\noindent \textbf{Response.}~In revision, we evaluate how ORAM protocols can
mitigate our attack in \S~\ref{subsec:oram}.
%\\\\
%\noindent \textit{Review~\#404B: Compare with other side-channel attacks (i.e.,
%  those not using the manifold)}
%
%\noindent \textbf{Response.}~\fixme{XXX}
\\\\
\noindent \textit{Review~\#404B: Evaluate the performance of countermeasure
  against different attacks and in presence of the white-box attacker}

\noindent \textbf{Response.}~Paragraph \textbf{Application Scope} in
\appx~\ref{sec:blind-appx} gives discussions on the application scope of our
proposed perception blinding. In particular, we clarified that perception
blinding is particularly designed against manifold learning-based SCA. It should
not be effective to mitigate other side channel attacks.

Perception blinding can mitigate the white-box attacker or incur high extra cost
(i.e., retraining a new model), depending on the knowledge a white-box attacker
has. We give corresponding discussions in paragraph \textbf{``White-Box''
  Attackers} in \appx~\ref{sec:blind-appx}.
%Alternatively, while we launch ``black-box'' attack where we assume zero
%knowledge on the victim \ms's implementation. In revision we also benchmarked a
%``white-box attacker''. When assessing to what extent ORAM can mitigate our
%attack, we actually launch a white-box attack to reconstruct images from side
%channel sub-traces made by critical functions (instead of the entire program
%executable) with known information leakage. Please refer to \S~\ref{subsec:oram}
%for details.
\\\\
\noindent \textit{Review~\#404B: Discuss how difficult would be to combine the
  proposed countermeasure with other countermeasures}

\noindent \textbf{Response.}~Thank you for the suggestion. Paragraph
\textbf{Application Scope} in \appx~\ref{sec:blind-appx} has clarified that
perception blinding is particularly designed for manifold learning-based SCA.
And perception blinding actually shows very promising results to mitigate our
proposed attack. It is unclear to us the reason to combine perception blinding
with other countermeasures. Nevertheless, we also present how other
countermeasures and various noise insertion schemes can influence our attack in
\S~\ref{subsec:oram} and \S~\ref{subsec:noise}, respectively.
\\\\
\noindent \textit{Review~\#404B: Improve threat model.}

\noindent \textbf{Response:}~Thank you for the advice.
In \textbf{Threat Model and Attack Scenarios} on Page 2, we have revised our
threat model, research assumption, and how side channels are acquired by
attackers. \\\\
\noindent \textit{Review~\#404C: Explain the choise for the blinding measure}

\noindent \textbf{Response.}~Thank you for the suggestion. We have extended
\S~\ref{subsec:design-defense} to clarify the requirement and usage of
perception blinding. We have also given more discussions about perception
blinding in \appx~\ref{sec:blind-appx}.
\\\\
\noindent \textit{Review~\#404C: p4: M_{I, O} = {(x, F(i)} and the sentence
  below: x is not defined}

\noindent \textbf{Response.}~We apologize for this typo. We have fixed it. $x$
should be $i$.
\\\\
\noindent \textit{Review~\#404C: I could not reach the code and data link
  (reference [3])}

\noindent \textbf{Response.}~Instead of using the Github anonymous URL service
(which could be unstable), we create an anonymous account for this project and
host all our code at \url{https://github.com/research-artifact/manifold-sca}. We
commit to maintain our released software for results verification and benefit
follow-up research.
\\\\
\noindent \textit{Review~\#404D: It is unclear to the reviewer how the blinding
  technique can be used in a real system.}

\noindent \textbf{Response.}~Thank you for the suggestion. We provided
\appx~\ref{sec:blind-appx} to elaborate on the usage of perception blinding,
discuss its application scope, and its effectiveness even in front of white-box
attackers.
\\\\
\noindent \textit{Review~\#404D: The paper should provide more details on how
  that traces are collected. In particular, how to overcome the cache hurdle.}

\noindent \textbf{Response.}~Thank you for pointing this out. We have clarified
this point in \appx~\ref{sec:attack-appendix} (for Pin logged trace) and
\appx~\ref{subsec:real-attack-details} (for side channels logged by \pp). On
page 2, we also highlight the key message in \textbf{Threat Model and Attack
  Scenarios}.
\\\\
\noindent \textit{Review~\#404D: In particular, how these specific traces were
  obtained and what the impact of the multiple caches is on trace quality.}

\noindent \textbf{Response.}~Thank you for the comment. We have answered how
traces were collected above.

Regarding real-world (noisy) scenarios and their impacts on our attack, we
benchmarked in total nine different scenarios. Particularly, given
that we launch \pp\ attack by pinning the victim process (e.g., \libjpeg) and
the \spy\ process on the same CPU core, we benchmark three real workloads by
launching 1) a \texttt{bzip2} software on the same core, 2) another victim
process processing a different input on the same core, and 3) another victim
process processing the same input on the same core. Since we have three \ms,
nine noise insertion schemes actually lead to 27 different evaluation settings.
Our attack manifest reasonably high accuracy for almost all settings. We give
further discussion on the noise resiliency of our attack in
\S~\ref{subsec:noise} and \appx~\ref{sec:noise}.
\\\\
\noindent \textit{Review~\#404D: It would be important to understand the quality
  of the attack/mitigation result relatively to related work. The authors should
  also look discuss other work that used autoencoders in the context of side
  channel attacks such as (although this prior work does not address the same
  objectives as this paper)}

\noindent \textbf{Response.}~Thank you for the comment. We have added
  these related works and present discussions accordingly.
\\\\
\noindent \textit{Review~\#404D: The paper needs some improvements in terms of
  writing.}

\noindent \textbf{Response.}~Thank you for pointing this out. We have fixed
those errors. During the revision phase, we have made major improvement on
writing. Please refer to \textbf{Formatting \& Writing \& Code Release} above
for details.
\\\\
\noindent \textit{Review~\#404E: Demonstrate the attack end-to-end, starting
  with an attacker generating the necessary trace data}

\noindent \textbf{Response.}~Thank you for the suggestion. In revision, we
benchmark userspace-only scenarios where attackers can launch
\pp\ attack~\cite{Tromer10} to log cache activities when \ms\ is processing a
secret input. We use Mastik~\cite{yarom2016mastik}, a micro-architectural
side-channel toolkit, to launch ``out-of-the-box'' \pp\ and log victim's L1I and
L1D cache activities. We pin victim process and \spy\ process on the same CPU
core; see attack details in \S~\ref{subsec:real-world} and
\appx~\ref{subsec:real-attack-details}.
\\\\
\noindent \textit{Review~\#404E: A related concern I have is that this work is
  not accurately placed in context with existing work in the security literature
  in side channel analysis. The related work section mentions various papers on
  cache-based side channel attacks to recover cryptographic key material, but
  those attacks have widely varying threat models, requirements, and outcomes.
  How does this paper fit in with that work, and how does it advance our
  understanding of the (lack of) security of our current systems?}

\noindent \textbf{Response.}~Thank you for the comment. In \textbf{Threat Model
  and Attack Scenarios} on Page 2, we have revised our threat model, research
assumption, and how side channels are acquired by attackers.

In general, the current paper includes two scenarios where attackers can either
log fine-grained cache line/cache bank/page table
information~\cite{xu2015controlled,yarom2017cachebleed,hahnel2017high,disselkoen2017prime},
or launch standard \pp\ attack in an end-to-end manner to log cache side
channels for media data reconstruction. We compare and discuss how our trace
encoder can smoothly process these two kinds of data in \appx~\ref{sec:input}.
We view that as an encouraging evidence to illustrate the generalization and
effectiveness of our attack under different scenarios.
\\\\
\noindent \textit{Review~\#404E: The paper presents a masking technique aimed at
  mitigating the proposed attack. The technique appears effective; however,
  there are sure to be viable attacks against it. A discussion of the weaknesses
  and limitations of the proposed masking technique would strengthen this
  paper.}

\noindent \textbf{Response.}~The perception blinding can only mitigate manifold
learning-based SCA toward \ms. It is not applicable to protect crypto software.
We elaborate on the usage of blinding in \appx~\ref{sec:blind-appx}. In
particular, we use two paragraphs, \textbf{Application Scope} and
\textbf{``White-Box'' Attackers}, to discuss the application scope, usage and
limitations of our proposed perception blinding.
%\\\\
%\noindent \textit{Review~\#404E: The paper demonstrates that given extensive
%  trace log information of media software, cross-modality manifold learning can
%  be used to reconstruct the original media data (text and images). This reads
%  to me more as a learning paper than a security paper. It's not clear what the
%  novelty is on the learning side, however. How does this fit in with prior work
%  to reconstruct media data outside of a security setting? Prior work to recover
%  images from system side data [111] seems to be the most closely related to
%  this work, but there is no comparison made to that work in the evaluation.
%  What other reconstruction work has been done, and how does this fit in?}
%
%\noindent \textbf{Response.}~\fixme{XXX}.




==> table_data.tex <==
\begin{table}[t]
  \caption{Quantitative evaluation results of Chest X-ray dataset in terms of
    Gaussian noise resiliency with $x=$(NA/0.2/0.5). We use cache line side
    channel.}
  \label{tab:xray-noise}
  \centering
\resizebox{1.0\linewidth}{!}{
  \begin{tabular}{l|c|c|c}
    \hline
     Disease & \textbf{Cardiomegaly} & \textbf{Consolidation} & \textbf{Atelectasis} \\
    \hline
     Precision & 0.74/0.72/0.66    & 0.76/0.74/0.74 & 0.83/0.80/0.72           \\
    \hline
     Recall    & 0.55/0.52/0.51    & 0.91/0.91/0.91 & 0.67/0.62/0.53           \\
    \hline
     F1 Score  & 0.63/0.61/0.57    & 0.82/0.81/0.81 & 0.75/0.70/0.61           \\
    \hline
  \end{tabular}
  }
\end{table}

\begin{table}[t]
  \caption{Quantitative evaluation results of Chest X-ray dataset in terms of
    zero replacement resiliency with $x=$(NA/20/50). We use cache line side
    channel.}
  \label{tab:xray-zero}
  \centering
\resizebox{1.0\linewidth}{!}{
  \begin{tabular}{l|c|c|c}
    \hline
     Disease   & \textbf{Cardiomegaly} & \textbf{Consolidation} & \textbf{Atelectasis} \\
    \hline
     Precision & 0.74/0.70/0.66      & 0.76/0.74/0.74       & 0.83/0.79/0.73    \\
    \hline
     Recall    & 0.55/0.53/0.51      & 0.91/0.90/0.92       & 0.67/0.60/0.53    \\
    \hline
     F1 Score  & 0.63/0.60/0.57      & 0.82/0.81/0.82       & 0.75/0.68/0.62    \\
    \hline
  \end{tabular}
  }
\end{table}

\begin{table}[t]
  \caption{Quantitative evaluation results of Chest X-ray dataset in terms of
    round shifting resiliency with $x=$(NA/10/100). We use cache line side
    channel.}
  \label{tab:xray-shift}
  \centering
\resizebox{1.0\linewidth}{!}{
  \begin{tabular}{l|c|c|c}
    \hline
     Disease   & \textbf{Cardiomegaly}  & \textbf{Consolidation} & \textbf{Atelectasis} \\
    \hline
     Precision & 0.74/0.74/0.74       & 0.76/0.75/0.75       & 0.83/0.85/0.86           \\
    \hline
     Recall    & 0.55/0.54/0.52       & 0.91/0.92/0.91       & 0.67/0.62/0.61           \\
    \hline
     F1 Score  & 0.63/0.62/0.61       & 0.82/0.82/0.83       & 0.75/0.71/0.71           \\
    \hline
  \end{tabular}
  }
\end{table}

\begin{table}[t]
  \caption{Quantitative evaluation results of Chest X-ray dataset in terms of
    random removal resiliency with $x=$(NA/20/50). We use cache line side
    channel.}
  \label{tab:xray-removal}
  \centering
\resizebox{1.0\linewidth}{!}{
  \begin{tabular}{l|c|c|c}
    \hline
     Disease   & \textbf{Cardiomegaly} & \textbf{Consolidation} & \textbf{Atelectasis} \\
    \hline
     Precision & 0.74/0.63/0.60      & 0.76/0.74/0.75       & 0.83/0.62/0.60    \\
    \hline
     Recall    & 0.55/0.42/0.42      & 0.91/0.88/0.89       & 0.67/0.44/0.44    \\
    \hline
     F1 Score  & 0.63/0.51/0.50      & 0.82/0.81/0.81       & 0.75/0.52/0.51    \\
    \hline
  \end{tabular}
  }
\end{table}

\begin{table}[t]
  \caption{Quantitative evaluation results of SC09 dataset in terms of four noise.}
  \label{tab:voice-robust}
  \centering
\resizebox{0.8\linewidth}{!}{
  \begin{tabular}{l|c|c|c}
    \hline
            & NA & $x$=20/0.2/10/20 & $x$=50/0.5/100/50 \\
    \hline
      \textbf{zero}  & 28.8\%  & 22.6\% & 17.9\% \\
    \hline
      \textbf{Noise} & 28.8\%  & 20.4\% & 17.0\% \\
    \hline
      \textbf{Shift} & 28.8\%  & 28.6\% & 26.3\% \\
    \hline
      \textbf{Removal} & 28.8\%  & 25.0\% & 24.5\% \\
    \hline
  \end{tabular}
  }
\end{table}

\begin{table}[t]
    \caption{Text data inference from noisy side channels. DDialog is short for
      DailyDialog.}
    \label{tab:text-noise}
    \centering
  \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l|c|c|c|c|c|c|c|c|c}
      \hline
        &  & \multicolumn{2}{|c|}{\textbf{Zero}} & \multicolumn{2}{|c|}{\textbf{Noise}} & \multicolumn{2}{|c}{\textbf{Shift}} & \multicolumn{2}{|c}{\textbf{Removal}} \\
      \hline
       \textbf{Weight} & NA            & 20 & 50       & 0.2 & 0.5       & 10 & 100       & 20 & 50\\
      \hline
       COCO & 42.6\%                   & 40.6\% & 35.8\% & 41.5\% & 34.9\% & 30.6\% & 31.8\% & 40.8\% & 40.7\%\\
      \hline
       DDialog & 37.4\%                & 36.7\% & 30.1\% & 35.5\% & 30.8\% & 25.6\% & 27.0\% & 32.8\% & 32.6\%\\
      \hline
    \end{tabular}
  }
   \vspace{-10pt}
  \end{table}

==> vulnerability.tex <==
\section{Vulnerability Localization Summary}
\label{sec:vulnerability}

This section localizes vulnerabilities identified in this research. We report the
assembly code line numbers. We use the default configuration to compile each
\ms, whose compiled executable file can be found in our released
repository~\cite{snapshot}. Hence, developers can use our reported information and
released executable files to localize and further patch relevant code fragments. 

